Dual-Resonator Organic Microcavities for Triplet-Triplet Annihilation Upconversion

Solid-state triplet-triplet annihilation upconversion offers a compelling route to harvest sub-bandgap photons to increase the efficiency of photovoltaics, but low sensitizer doping required to suppress non-radiative aggregation quenching severely restricts light absorption. Here, we present a dual-resonator planar silver microcavity housing a thermally co-evaporated rubrene:palladium phthalocyanine (PdPC) active layer designed to simultaneously enhance triplet-sensitizer absorption and out-couple upconverted emission. By aligning a dispersive cavity mode with the PdPC absorption peak at $32^\circ$, we achieve a 12-fold enhancement in absorptance at 665 nm. This absorption boost, combined with directional outcoupling through a second cavity mode, outweighs cavity-induced reabsorption losses to yield a 22-fold peak and 4.5-fold integrated enhancement in detected upconversion emission. Overall, this work highlights the potential of microcavity integration to substantially enhance solid-state upconversion performance across low-intensity optoelectronic applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "pdflatex -interaction=batchmode -shell-escape \"$_[0]\"" );
    }
}
